DeepGG: a Deep Graph Generator

Learning distributions of graphs can be used for automatic drug discovery, molecular design, complex network analysis, and much more. We present an improved framework for learning generative models of graphs based on the idea of deep state machines. To learn state transition decisions we use a set of graph and node embedding techniques as memory of the state machine. Our analysis is based on learning the distribution of random graph generators for which we provide statistical tests to determine which properties can be learned and how well the original distribution of graphs is represented. We show that the design of the state machine favors specific distributions. Models of graphs of size up to 150 vertices are learned. Code and parameters are publicly available to reproduce our results.

==> content/figure-degree-distribution-kde-barabasi-albert.tex <==
\begin{figure*}
  \begin{minipage}[c]{0.5\linewidth}
    \includegraphics[width=\linewidth]{\visBasePath degree-distribution-kde-barabasi-albert.png}
  \end{minipage}\hfill
  \begin{minipage}[c]{0.49\linewidth}
    \caption{
      For \textit{DeepGG} instances trained on scale-free graphs of the Barabasi-Albert model we observe a similar degree distribution between generated graphs and the BA-model.
      This goes along with the experiment of \cite{li2018learning} in which Li et al. report a small KL-divergence of 0.0013 between three instances of \textit{DGMG} and B-A-graphs.
      However, we observe that at least \textit{DeepGG} does often not come close to the degree distribution of the WS- or ER-model and we have a suspicion that both \textit{DGMG} and \textit{DeepGG} favor scale-free networks.
    }
    \label{fig:degree-distribution-kde}
  \end{minipage}
\end{figure*}


==> content/quotes.tex <==


% misc or early work, representation learning
The graph neural network model \cite{scarselli2008graph}
``the GNN is an extension of both recursive neural networks and randomwalk models and that it retains their characteristics''

Graph attention networks \cite{velivckovic2017graph}

Grammar Variational Autoencoder \cite{kusner2017grammar}
``propose to directly incorpo-rate knowledge about the structure of discrete data usingagrammar.''
``pro-pose thegrammar variational autoencoder(GVAE) whichencodes and decodes directly from and to these parse trees''
technique: autoencoder


Learning graphical state transitions \cite{johnson2016learning}
Gated Graph Transformer Neural Network model

Graph convolution \cite{kipf2016semi}

Neural message passing for quantum chemistry + Message passing framework \cite{gilmer2017neural}


% Kronecker fit
Scalable modeling of real graphs using kronecker multiplication \cite{leskovec2007scalable}
``Kronecker model can generate graphs that obey many of the patterns found in real graphs. More-over, we present KronFit, a fast and scalable algorithm for fitting Kronecker graphs by using maximum likelihood. ''
``We evaluate the probability that G is a realization of P. The task is to find such $\theta$ that has the highest probability of generating G.''
``we  describe  a  Metropolis  algorithm  to simulate  draws  from  the  permutation  distribution''
technique: bayesian, maximum likelihood, probabilistic model parameter fit, metropolis sampling

Kronecker Graphs: An Approach to Modeling Networks \cite{leskovec2010kronecker}
``In Kronecker graphs permuta-tions of the parameter matrix $\Theta$ all have the same like-lihood. This means that the maximum likelihood opti-mization problem is not convex, but rather has severalglobal minima.``
``Sampling: Similarly,if we want a realistic sample of the real graph, we coulduse a smaller exponent in the Kronecker exponentia-tion, like $\Theta\_{[k-1]}$.''


% generative

GraphRNN: Generating Realistic Graphs with Deep Auto-regressive Models \cite{you2018graphrnn}
``here we address the above challenges and present Graph Recurrent Neural Networks(GraphRNN),a  scalable  framework  for  learning  generative  models  of graphs. GraphRNN models a graph in an autoregressive (orrecurrent) manner—as a sequence of additions of new nodesand edges—to capture the complex joint probability of allnodes and edges in the graph''
``Thus, instead of learningp(G), whose sample space cannotbe easily characterized, we sample the auxiliary $\pi$ to get theobservations ofS$\pi$ and learnp(S $\pi$ ), which can be modeledautoregressively due to the sequential nature ofS$\pi$ ''
technique: RNN

Learning Deep Generative Models of Graphs \cite{li2018learning}
``our goal in this paper is to learn and represent unconditional or conditional densities on a space of graphs given a representative set of graphs''
technique: state-machine with graph-message-passing and log-prop-backprop modules


Efficient graph generation with graph recurrent attention networks \cite{liao2019efficient}
`` On the other hand,previous work that exploits general graph structures using graph neural networks (GNNs) [21] do notscale well, with a maximum size of the generated graphs not exceeding 100 nodes''
``Without using GNNs in the loop, these models can scale up significantly, to generate graphs withhundreds of nodes. However, the GraphRNN model has some important limitations: (1) the numberof generation steps in the full GraphRNN is still very large (O(N2)for the best model, whereNisthe number of nodes); (2) due to the sequential ordering, two nodes nearby in the graph could be farapart in the generation process of the RNN, which presents significant bottlenecks in handling suchlong-term dependencies''


Graphite: Iterative generative modeling of graphs \cite{grover2018graphite}

Discriminative embeddings of latent variable models for structured data \cite{dai2016discriminative}

Graphgan: Graph representation learning with generative adversarial nets \cite{wang2018graphgan}


% generative & applied

Molecular generation with recurrent neural networks (RNNs) \cite{bjerrum2017molecular}
technique: RNN

Generative Recurrent Networks for De Novo Drug Design \cite{gupta2018generative}
technique: RNN

Junction tree variational autoencoder for molecular graph generation \cite{jin2018junction}

Improving chemical autoencoder latent space and molecular de novo generation diversity with heteroencoders \cite{bjerrum2018improving}
``it is shown that the choice of chemical representation, such as strings from the simplified molecular-input line-entry system (SMILES), has a large influence on the properties of the latent space''
``explored to what extent translating between different chemical representations influences the latent space similarity to the SMILES strings or circular fingerprints''

Graph Convolutional Policy Network for Goal-Directed Molecular Graph Generation \cite{you2018graph}
technique: ???

DeepChemStable: Chemical Stability Prediction with an Attention-Based Graph Convolution Network \cite{li2019deepchemstable}


